A New Metric on Symmetric Group and Applications to Block Permutation Codes

Permutation codes have received a great attention due to various applications. For different applications, one needs permutation codes under different metrics. The generalized Cayley metric was introduced by Chee and Vu [4] and this metric includes several other metrics as special cases. However, the generalized Cayley metric is not easily computable in general. Therefore the block permutation metric was introduced by Yang et al. [22] as the generalized Cayley metric and the block permutation metric have the same magnitude. However, the block permutation metric lacks the symmetry property which restricts more advanced algebraic tools to be involved. In this paper, by introducing a novel metric closely related to the block permutation metric, we build a bridge between some advanced algebraic methods and codes in the block permutation metric. More specifically, based on some techniques from algebraic function fields originated in [19], we give an algebraic-geometric construction of codes in the novel metric with reasonably good parameters. By observing a trivial relation between the novel metric and block permutation metric, we then produce non-systematic codes in block permutation metric that improve all known results given in [21, 22]. More importantly, based on our non-systematic codes, we provide an explicit and systematic construction of codes in block permutation metric which improves the systematic result shown in [22]. In the end, we demonstrate that our codes in the novel metric itself have reasonably good parameters by showing that our construction beats the corresponding Gilbert-Varshamov bound.

==> sn-sample-bib.tex <==
\begin{thebibliography}{99}
\bibitem{5}
S. Buzaglo, T. Etzion. ``Bounds on the Size of Permutation Codes With the Kendall $\tau$-Metric." \emph{IEEE Transactions on Information Theory} 61.6 (2015): 3241-3250.
\bibitem{11} S. Buzaglo, E. Yaakobi, T. Etzion, J. Bruck. ``Systematic error-correcting codes for permutations and multi-permutations." \emph{IEEE Transactions on Information Theory} 62.6 (2016): 3113-3124.
\bibitem{12}
W. Chu, C. Colbourn, and P. Dukes. ``Constructions for permutation codes in powerline communications." \emph{Designs, Codes and Cryptography} 32.1 (2004): 51-64.
\bibitem{3}
Y. Chee, V. K. Vu. ``Breakpoint analysis and permutation codes in generalized Kendall tau and Cayley metrics." \emph{2014 IEEE International Symposium on Information Theory.} IEEE, 2014.
\bibitem{13}
C. Colbourn, T. Klove, and A. Ling. ``Permutation arrays for powerline communication and mutually orthogonal Latin squares." \emph{IEEE Transactions on Information Theory} 50.6 (2004): 1289-1291.
\bibitem{17}
C. Ding, F. Fu, T. Klove, and V. Wei. ``Constructions of permutation arrays." \emph{IEEE Transactions on Information Theory} 48.4 (2002): 977-980.
\bibitem{1}
M. Deza, S.A. Vanstone. ``Bounds for permutation arrays." \emph{Journal of Statistical Planning and Inference} 2.2 (1978): 197-209.
\bibitem{2}
P. Frankl, M. Deza. ``On the maximum number of permutations with given maximal or minimal distance." \emph{Journal of Combinatorial Theory, Series A} 22.3 (1977): 352-360.
\bibitem{15}
F. Fu, T. Klove. ``Two constructions of permutation arrays." \emph{IEEE Transactions on Information Theory} 50.5 (2004): 881-883.

\bibitem{7}
F. Farnoud, O. Milenkovic. ``Multipermutation codes in the Ulam metric for nonvolatile memories." \emph{IEEE Journal on Selected Areas in Communications} 32.5 (2014): 919-932.
\bibitem{6}
F. Farnoud, V. Skachek and O. Milenkovic. ``Error-correction in flash memories via codes in the Ulam metric." \emph{IEEE Transactions on Information Theory} 59.5 (2013): 3003-3020.
\bibitem{14}
F. Gao, Y. Yang, and G. Ge. ``An improvement on the Gilbert-Varshamov bound for permutation codes." \emph{IEEE transactions on information theory} 59.5 (2013): 3059-3063.
\bibitem{4}
F. G\"{o}loglu, J. Lember, A. Riet and V. Skachek. ``New bounds for permutation codes in Ulam metric." \emph{2015 IEEE International Symposium on Information Theory (ISIT).} IEEE, 2015.
\bibitem{Jin}
L. Jin. ``A Construction of Permutation Codes From Rational Function Fields and Improvement to the Gilbert-Varshamov Bound. \emph{IEEE transactions on information theory}, vol. 62, no. 1, pp. 159-162, Jan. 2016.
\bibitem{jcta2002}
A. N. Myers. ``Counting permutations by their rigid patterns." \emph{Journal of Combinatorial Theory, Series A }99.2 (2002): 345-357.
\bibitem{16}
T. Michael, A. Vardy, and J. Verstra\"{e}te. ``Asymptotic improvement of the Gilbert-Varshamov bound on the size of permutation codes." arXiv preprint arXiv:1311.4925 (2013).

\bibitem{NX} H. Niederreiter and C. Xing. {\it Rtional points on curves over finite fields.} Cambridge University Press, LMS 285, 2001.

\bibitem{GTM254}
H. Stichtenoth. ``Algebraic function fields and codes." GTM 254, Springer, New York, 2009.
\bibitem{e}
D. H. Smith, Roberto Montemanni. ``A new table of permutation codes." \emph{Designs, Codes and Cryptography} 63.2 (2012): 241-253.
\bibitem{8}
X. Wang, Y. Zhang and G. Ge. ``New bounds of permutation codes under Hamming metric and Kendall's $\tau$-metric." \emph{Designs, Codes and Cryptography} 85.3 (2017): 533-545.
\bibitem{chaoping2002}
C. Xing.  ``Constructions of codes from residue rings of polynomials."  \emph{IEEE Transactions on Information Theory} 48.11 (2002): 2995-2997.
\bibitem{chaoping2004}
C. Xing. ``Linear codes from narrow ray class groups of algebraic curves." \emph{IEEE Transactions on Information Theory} 50.3 (2004): 541-543.
\bibitem{Xu}
Z. Xu, Y. Zhang and G. Ge. ``New theoretical bounds and constructions of permutation codes under block permutation metric. \emph{Designs, Codes and Cryptography} 87 (2019), no. 11, 2625-2637.
\bibitem{Yang}
S. Yang, C. Schoeny and L. Dolecek. ``Theoretical Bounds and Constructions of Codes in the Generalized Cayley Metric. \emph{IEEE Transactions of Information Theory}, vol. 65, no. 8, pp. 4746-4763, Aug. 2019.
\bibitem{9}
Y. Zhang, and G. Ge. ``Snake-in-the-Box Codes for Rank Modulation Under Kendall's $\tau $-Metric." \emph{IEEE Transactions on Information Theory} 62.1 (2015): 151-158.


\end{thebibliography}


